Hypergraph Convolutional Networks for Weakly-Supervised Semantic Segmentation

Semantic segmentation is a fundamental topic in computer vision. Several deep learning methods have been proposed for semantic segmentation with outstanding results. However, these models require a lot of densely annotated images. To address this problem, we propose a new algorithm that uses HyperGraph Convolutional Networks for Weakly-supervised Semantic Segmentation (HyperGCN-WSS). Our algorithm constructs spatial and k-Nearest Neighbor (k-NN) graphs from the images in the dataset to generate the hypergraphs. Then, we train a specialized HyperGraph Convolutional Network (HyperGCN) architecture using some weak signals. The outputs of the HyperGCN are denominated pseudo-labels, which are later used to train a DeepLab model for semantic segmentation. HyperGCN-WSS is evaluated on the PASCAL VOC 2012 dataset for semantic segmentation, using scribbles or clicks as weak signals. Our algorithm shows competitive performance against previous methods.

==> old_stuff.tex <==
\begin{table}[]
\centering
\caption{Accuracy of HyperGCN-WSS and other methods in the validation set of PASCAL VOC. S: Scribbles. C: Clicks.}
\label{tbl:comparisons}
\begin{tabular}{r|ccc}
\hline
Method            & \begin{tabular}[c]{@{}c@{}}Weak\\ Signal\end{tabular} & CRF & mIoU (\%) \\
\hline
ScribbleSup \cite{lin2016scribblesup} & S & \checkmark & $63.1$ \\
RAWKS \cite{vernaza2017learning} & S & \checkmark & $61.4$ \\
NormalizedCutLoss \cite{tang2018normalized} & S & - & $60.5$ \\
%NormalizedCutLoss \cite{tang2018normalized} & S & \checkmark & $65.1$ \\
GraphNet \cite{pu2018graphnet} & S & - & $63.3$ \\
\hline
HyperGCN-WSS (\textcolor{red}{ours}) & S & - & $65.3$ \\
HyperGCN-WSS (\textcolor{red}{ours}) & C & - & $\textbf{65.4}$ \\
\hline
\end{tabular}
\end{table}
